Is Perfect Filtering Enough Leading to Perfect Phase Correction for dMRI data?

Being complex-valued and low in signal-to-noise ratios, magnitude-based diffusion MRI is confounded by the noise-floor that falsely elevates signal magnitude and incurs bias to the commonly used diffusion indices, such as fractional anisotropy (FA). To avoid noise-floor, most existing phase correction methods explore improving filters to estimate the noise-free background phase. In this work, after diving into the phase correction procedures, we argue that even a perfect filter is insufficient for phase correction because the correction procedures are incapable of distinguishing sign-symbols of noise, resulting in artifacts (\textit{i.e.}, arbitrary signal loss). With this insight, we generalize the definition of noise-floor to a complex polar coordinate system and propose a calibration procedure that could conveniently distinguish noise sign symbols. The calibration procedure is conceptually simple and easy to implement without relying on any external technique while keeping distinctly effective.

==> Fig/pc_real/real2/Fig9a.tex <==
\tikzset{
		/tpic/options/.style = {
			width =\iwidth,
			height=\iheight,
			scale=1.05,
			xloc=0.5,
			yloc=0.5,
			angle=0,
			color=white,
			label={}
		}
}
\begin{tabular}{ccccccc} 
		%\columnText{$0\,\text{s/mm}^2$}     \tpic[options]{TV}   &  \tpic[options]{TV_real_noise}   &  \tpic[options]{CF}  &  \tpic[options]{CF_real_noise}  & \tpic[options]{MPPCA_real}  & \tpic[options]{MPPCA_real_noise}  &  \tpic[options]{data}  \vspace{-4mm}  \\
		%\columnText{$750\,\text{s/mm}^2$}   \tpic[options]{TV2}  &  \tpic[options]{TV_real_noise2}  &  \tpic[options]{CF2} &  \tpic[options]{CF_real_noise2} & \tpic[options]{MPPCA_real2} & \tpic[options]{MPPCA_real_noise2} &  \tpic[options]{data2} \vspace{-4mm}  \\ 	
		   %\\
		\tpic[options]{../real/TV4}  &  \tpic[options]{../real/TV_real_noise4}  &  \tpic[options]{../real/CF4} &  \tpic[options]{../real/CF_real_noise4} & \tpic[options]{../real/MPPCA4}      & \tpic[options]{../real/MPPCA_real_noise4} &  \tpic[options]{../real/data4} 
		\vspace{-2mm} 
		\\
		\tpic[options]{../real/tv_r}  &  \tpic[options]{../real/tv_n_r}  &  \tpic[options]{../real/cf_r} &  \tpic[options]{../real/cf_n_r} & \tpic[options]{../real/mppca_r} & \tpic[options]{../real/mppca_n_r} &  \tpic[options]{../real/data_r}  
		\vspace{-2mm}
		\\  
		\tiny{TV} &  \tiny{\textbf{\textcolor{red}{TV-new}}}             &  \tiny{CF}     &  \tiny{\textbf{\textcolor{red}{CF-new}}}            & \tiny{MPPCA}          & \tiny{\textbf{\textcolor{red}{MPPCA-new}}}            &  \tiny{MAG}
\end{tabular}



	
%\end{document}


==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/FA/F10.tex <==
\usetikzlibrary{backgrounds,arrows}
\usetikzlibrary{arrows,shapes,chains}
\usetikzlibrary{automata, chains, decorations.pathmorphing, positioning}
\usetikzlibrary{shapes.geometric, arrows,shapes.multipart}
\usetikzlibrary{fadings}


\let\iwidth\relax
\let\iheight\relax
\let\rowspace\relax
\newlength{\iwidth}
\newlength{\iheight}
\newlength{\rowspace}
\setlength{\iwidth}{0.1\textwidth}
\setlength{\iheight}{1.0\iwidth}
\setlength{\rowspace}{0pt} 





\setlength{\tabcolsep}{1.5pt}

\newlength{\colorbarlength}
\setlength{\colorbarlength}{0.4\iheight}

\newcommand{\columnText}[1]{
	\begin{tikzpicture}[baseline,trim right=5pt]
		\node[rotate=90] at (0.05\iwidth, 0.5\iheight) {\tiny{#1}};
	\end{tikzpicture}
} 

\newlength{\gbarlength}
\newcommand\gBar[2]{		
	\begin{tikzpicture} %[baseline=(current bounding box.south)]
		\node (bar) {\pgfuseshading{g1}}; 
		\node [below=0mm of bar] {\scriptsize{#1}};
		\node [above=-0.3mm of bar] {\scriptsize{#2}};
	\end{tikzpicture}
} 	

\newcommand\colorBar[2]{		
	\begin{tikzpicture} %[baseline=(current bounding box.south)]
		\node (bar) {\pgfuseshading{spectrum1}}; 
		\node [below=0mm of bar] {\scriptsize{#1}};
		\node [above=-0.3mm of bar] {\scriptsize{#2}};
	\end{tikzpicture}
}     


\begin{figure}[t] 
\centering
    \begin{tikzpicture}
             \pgfdeclareverticalshading{spectrum1}{.16cm}{
             	rgb(0)=(0,0,0); 
             	rgb(0.13\colorbarlength)=(0,0,1); 
             	rgb(0.43\colorbarlength)=(0,1,1); 
             	rgb(0.65\colorbarlength)=(0,1,0); 
             	rgb(0.86\colorbarlength)=(1,1,0); 
             	rgb(1.17\colorbarlength)=(1,0,0); 
             	rgb(1.30\colorbarlength)=(1,1,1)
             }
        \node(dum) {\subimport{Fig/FA/}{syn0_1.tex}};
        \node(cb) [above right = -1.8cm and -0.3cm of dum] {\colorBar{${0}$}{${1}$}};
             \pgfdeclareverticalshading{spectrum1}{.16cm}{ 
                	rgb(0)=(1,1,1);
                	rgb(0.1\colorbarlength)=(0,0,1);
                	rgb(0.3\colorbarlength)=(0,1,0);                	
                	rgb(0.5\colorbarlength)=(0,0,0);  
                	rgb(0.55\colorbarlength)=(0,0,0);	
                	rgb(0.6\colorbarlength)=(0,0,0);                	
                	rgb(0.8\colorbarlength)=(1,1,0);
                	rgb(1.0\colorbarlength)=(1,0,0) %0.15               	 
                }
        \node(db) [below right = -1.6cm and -2cm of dum] {\colorBar{${-0.4}$}{${0.4}$}};
    \end{tikzpicture}
    \\
    %\vspace{-0.4cm}
    \caption{ Visual comparison on synthetic data. Top: FA maps; Bottom: Error maps.}%purple
	\label{fig3}
\end{figure}


==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/FA/F11.tex <==
\usetikzlibrary{backgrounds,arrows}
\usetikzlibrary{arrows,shapes,chains}
\usetikzlibrary{automata, chains, decorations.pathmorphing, positioning}
\usetikzlibrary{shapes.geometric, arrows,shapes.multipart}
\usetikzlibrary{fadings}


\let\iwidth\relax
\let\iheight\relax
\let\rowspace\relax
\newlength{\iwidth}
\newlength{\iheight}
\newlength{\rowspace}
\setlength{\iwidth}{0.11\textwidth}
\setlength{\iheight}{1.0\iwidth}
\setlength{\rowspace}{0pt}



\tikzset{
	/tpic/options/.style = {
		width=\iwidth,
		height=\iheight,
		scale=1.05,
		xloc=0.5,
		yloc=0.5,
		angle=0,
		color=white,
		label={}
	}
}

\setlength{\tabcolsep}{1.5pt}


\setlength{\colorbarlength}{0.4\iheight}
\pgfdeclareverticalshading{spectrum1}{.20cm}{ %0.05\colorbarlength
	rgb(0)=(0,0,0); 
	rgb(0.13\colorbarlength)=(0,0,1); 
	rgb(0.43\colorbarlength)=(0,1,1); 
	rgb(0.65\colorbarlength)=(0,1,0); 
	rgb(0.86\colorbarlength)=(1,1,0); 
	rgb(1.17\colorbarlength)=(1,0,0); 
	rgb(1.30\colorbarlength)=(1,1,1)
}

\begin{figure}[t] 
\centering
    	\begin{tikzpicture}
    	    \node(dum) {\subimport{Fig/FA/}{real.tex}};
    	    \node(cb)  [ above right = -1.9cm and -0.3 cm of dum]  {\colorBar{${0}$}{${1}$}};
    	    %\node(cb1) [below right = -2.3cm and -2.2 cm of dum]  {\colorBar{${0}$}{${1}$}};
        \end{tikzpicture} \\
        %\vspace{-5mm}
    \caption{ FA maps obtained by phase correction without and with the calibration. Artifacts are significantly mitigated for all three filtering methods, while the FA values in corpus callosum are increased properly, after using calibration. }
	\label{fig5}
\end{figure}


==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/FA/Syn0_1.tex <==
\tikzset{
	/tpic/options/.style = {
		width=\iwidth,
		height=\iheight,
		scale=1.05,
		xloc=0.5,
		yloc=0.5,
		angle=0,
		color=white, 
		label={}
	}
}
	\begin{tabular}{ccccccccc}
		\columnText{FA maps} &
		\tpic[options]{sim/fa_tv} & \tpic[options]{sim/fa_tv_500} & \tpic[options]{sim/fa_cf} & \tpic[options]{sim/fa_cf_500} &
		\tpic[options]{sim/fa_mppca}   &  \tpic[options]{sim/fa_mppca_500} & \tpic[options]{sim/fa_mag_500} &
		\tpic[options]{sim/fa_MAG_nf} \vspace{-2mm}  
		\\					
		[0.6\rowspace] & \tiny{TV} & \tiny{\textbf{\textcolor{red}{TV-new}}} & \tiny{CF} & \tiny{\textbf{\textcolor{red}{CF-new}}} & \tiny{MPPCA}  & \tiny{\textcolor{red}{\textbf{MPPCA-new}}} & \tiny{MAG}  &  \tiny{Ground Truth} 
		\vspace{-2mm}  
		\\
		\vspace{-2mm} 
		\columnText{Error maps} &
		\tpic[options]{res/res_tv_real} & \tpic[options]{res/res_cf_real} &
		\tpic[options]{res/res_mppca_real}  & \tpic[options]{res/res_tv_real_new} & \tpic[options]{res/res_cf_real_new} & \tpic[options]{res/res_mppca_real_new} & \tpic[options]{res/res_mag_final} 		&
		\\
			[0.6\rowspace] & \tiny{TV} & \tiny{\textbf{\textcolor{red}{TV-new}}} & \tiny{CF} & \tiny{\textbf{\textcolor{red}{CF-new}}} & \tiny{MPPCA}  & \tiny{\textcolor{red}{\textbf{MPPCA-new}}} & \tiny{MAG} 
		\vspace{-2mm} 
		%\\
		%[0.6\rowspace] & \scriptsize{TV} & \scriptsize{CF} & \scriptsize{MPPCA} & \scriptsize{TV new} & \scriptsize{CF new} & \scriptsize{MPPCA new} & \scriptsize{MAG} &
	\end{tabular}


	


==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/FA/real.tex <==
\tikzset{
	/tpic/options/.style = {
		width=\iwidth,
		height=\iheight,
		scale=1.05,
		xloc=0.5,
		yloc=0.5,
		angle=0,
		color=white,
		label={}
	} 
}
	\begin{tabular}{cccccccc}
		\tpic[options]{real/fa_TV} & \tpic[options]{real/fa_TV_1} &\tpic[options]{real/fa_CF} & \tpic[options]{real/fa_CF_1} & 		\tpic[options]{real/fa_MPPCA} &   \tpic[options]{real/fa_MPPCA_1} &		\tpic[options]{real/fa_MAG}  
	\vspace{-2mm}
		\\		
	 \tiny{TV} & \tiny{\textbf{\textcolor{red}{TV-new}}} & \tiny{CF} & \tiny{\textbf{\textcolor{red}{CF-new}}} &  \tiny{MPPCA} & \tiny{\textbf{\textcolor{red}{MPPCA-new}}} & \tiny{MAG} 
 	 	   % real/fa_MAG3
	%	\\
		% [0.6\rowspace] & \scriptsize{TV} & \scriptsize{CF} & \scriptsize{MPPCA}  
	\end{tabular}
 


==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/curves.tex <==
\begin{figure} [t]
	% Use the relevant command to insert your figure file.
	% For example, with the graphicx package use	
	\centering
	\subfigure{
		\label{fig:mae}
		\subimport{Fig/}{mae.tex} 
	}
	\hspace{1mm}
	\subfigure{
		\label{fig:me}
		\subimport{Fig/}{me.tex}
	}
    \\
\definecolor{mycolor1}{rgb}{0.98820,0.61570,0.60390}%
\definecolor{mycolor2}{rgb}{0.97650,0.80390,0.67840}%
\definecolor{mycolor3}{rgb}{0.78430,0.78430,0.66270}%
\definecolor{mycolor4}{rgb}{0.51370,0.68630,0.60780}%
\vspace{-0.4cm}
	\ref{legend:CompMae}
	\\
	%\vspace{-0.4cm}
	\caption{Quantitative comparison on the synthetic data. (a) MAE on each DW image (volume), and (b) ME of each slice on FA maps.} % \textbf{}
	\label{fig:curves}       % Give a unique label
\end{figure}



==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/mae.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\definecolor{mycolor1}{rgb}{0.98820,0.61570,0.60390}%
\definecolor{mycolor2}{rgb}{0.97650,0.80390,0.67840}%
\definecolor{mycolor3}{rgb}{0.78430,0.78430,0.66270}%
\definecolor{mycolor4}{rgb}{0.51370,0.68630,0.60780}%
%
\begin{tikzpicture}

\begin{axis}[%
width=1.9in,   
height=0.9in,
at={(0.758in,0.481in)},
scale only axis,
xmin=0,
xmax=70,
xlabel style={at={(axis description cs:.5,.1)}, font=\color{white!15!black}},
xlabel={Volume Index},
ymin=209,
ymax=220,
ylabel style={at={(axis description cs:0.1,.5)}, font=\color{white!15!black}},
%
ylabel={(a) MAE},
axis background/.style={fill=white},
axis x line*=bottom,
axis y line*=left,
%xmajorgrids,
ymajorgrids,
label style={font=\tiny},
tick label style={font=\tiny},
legend columns=6,
legend style={at={(0.177,0.471)}, font=\tiny, anchor=south west, legend cell align=left,  fill=none, draw=none}, legend to name={legend:CompMae},
clip bounding box=upper bound 
]

\addplot [color=blue, dashed, mark size=1pt, mark repeat=20, mark=square*, mark options={solid, fill=blue, blue}]
  table[row sep=crcr]{%
1	212.188549912991\\
2	211.279205414257\\
3	210.951383102489\\
4	211.020464626282\\
5	211.590008896388\\
6	211.670281884586\\
7	211.143250138422\\
8	211.207145975721\\
9	211.693588659646\\
10	211.555204441927\\
11	211.344325738214\\
12	213.307741039905\\
13	212.628704661254\\
14	213.340319779002\\
15	213.093919031551\\
16	213.40904620916\\
17	212.248022457678\\
18	212.936626698123\\
19	213.090936397315\\
20	213.058859670108\\
21	212.927654921914\\
22	212.465616351255\\
23	212.64908426098\\
24	212.255643651846\\
25	212.619781674811\\
26	212.505258566164\\
27	212.899409288106\\
28	215.170330491555\\
29	213.787787162281\\
30	214.474539653611\\
31	213.996842000295\\
32	213.543304901624\\
33	214.519169613092\\
34	215.717090013253\\
35	214.447752275915\\
36	213.348338707628\\
37	214.962854418806\\
38	215.652201626577\\
39	214.133643766733\\
40	215.034907633518\\
41	215.158388041714\\
42	215.320828092079\\
43	215.350635644852\\
44	214.14504990001\\
45	215.827972057348\\
46	213.997479917625\\
47	215.586504122907\\
48	214.083419790088\\
49	215.128162492893\\
50	215.244529780817\\
51	215.031905240984\\
52	214.618525121918\\
53	214.018061327788\\
54	214.517063994236\\
55	215.308242700758\\
56	215.068376213877\\
57	214.043604086681\\
58	214.912998159767\\
59	214.457744932608\\
60	213.913414063959\\
61	215.114571186664\\
62	213.904125948818\\
63	215.122965487326\\
64	214.278039853275\\
65	214.748513865597\\
66	213.679599739302\\
67	214.595563456979\\
68	215.307601203773\\
69	213.823229064137\\
};
\addlegendentry{TV}

\addplot [color=blue, mark size=1pt, mark repeat=20, mark=square*, mark options={solid, fill=blue, blue}]
table[row sep=crcr]{%
	1	212.132231901948\\
	2	211.208741212705\\
	3	210.884789177361\\
	4	210.966872687536\\
	5	211.508260514975\\
	6	210.779510050571\\
	7	210.32938884458\\
	8	210.192760214077\\
	9	210.865637683425\\
	10	210.461584265288\\
	11	210.636081500257\\
	12	212.154524928208\\
	13	211.540967841804\\
	14	211.959674942707\\
	15	212.077038106832\\
	16	212.040260314077\\
	17	210.917313980388\\
	18	211.578736796585\\
	19	211.712230971529\\
	20	211.822441117304\\
	21	211.76424737855\\
	22	211.593586410876\\
	23	211.559841885901\\
	24	211.455454444705\\
	25	211.457597373607\\
	26	211.705663778806\\
	27	211.742673742724\\
	28	213.801373595638\\
	29	212.342187376233\\
	30	212.915047789709\\
	31	212.428386207751\\
	32	212.008993108053\\
	33	212.906402680938\\
	34	214.253511718814\\
	35	212.902726964228\\
	36	211.885299352655\\
	37	213.449923865183\\
	38	214.237593577076\\
	39	212.53081963774\\
	40	213.557012847033\\
	41	213.659302477608\\
	42	213.871220196215\\
	43	213.941472375611\\
	44	212.594298965339\\
	45	214.490916196226\\
	46	212.595503229985\\
	47	214.107507694445\\
	48	212.562659357\\
	49	213.756970464004\\
	50	213.756249043657\\
	51	213.57998795854\\
	52	213.299031673758\\
	53	212.777707325431\\
	54	213.116548399927\\
	55	213.790224212723\\
	56	213.557902799861\\
	57	212.495000190661\\
	58	213.323246516896\\
	59	212.938681028557\\
	60	212.473851594947\\
	61	213.698650614974\\
	62	212.382990656714\\
	63	213.667851839227\\
	64	212.710114199804\\
	65	213.307683494495\\
	66	212.05046172293\\
	67	212.958000615398\\
	68	213.730359399003\\
	69	212.330518072561\\
};
\addlegendentry{\textbf{\textcolor{red}{TV-new}}}

\addplot [color=green, dashed, mark size=1pt, mark repeat=20, mark=triangle, mark options={solid, fill=green, green}]
  table[row sep=crcr]{%
1	212.106536865234\\
2	211.531753540039\\
3	211.197891235352\\
4	211.188430786133\\
5	211.746231079102\\
6	211.885559082031\\
7	211.337539672852\\
8	211.606750488281\\
9	211.99153137207\\
10	211.679718017578\\
11	211.510955810547\\
12	213.640319824219\\
13	212.875534057617\\
14	213.548614501953\\
15	213.617538452148\\
16	213.578491210938\\
17	212.551284790039\\
18	213.257736206055\\
19	213.429153442383\\
20	213.377731323242\\
21	213.306304931641\\
22	212.88313293457\\
23	213.111877441406\\
24	212.491256713867\\
25	212.962554931641\\
26	212.756851196289\\
27	213.330123901367\\
28	215.326904296875\\
29	214.007232666016\\
30	214.630981445313\\
31	214.290237426758\\
32	213.662475585938\\
33	214.705108642578\\
34	215.922760009766\\
35	214.791519165039\\
36	213.434997558594\\
37	215.33171081543\\
38	215.84992980957\\
39	214.435150146484\\
40	215.274658203125\\
41	215.223678588867\\
42	215.489379882813\\
43	215.681198120117\\
44	214.378448486328\\
45	215.982284545898\\
46	214.124145507813\\
47	216.02180480957\\
48	214.178756713867\\
49	215.321166992188\\
50	215.373977661133\\
51	215.477981567383\\
52	214.651947021484\\
53	214.153610229492\\
54	214.920379638672\\
55	215.447052001953\\
56	215.283309936523\\
57	214.174926757813\\
58	214.918487548828\\
59	214.558624267578\\
60	214.390991210938\\
61	215.288497924805\\
62	214.275253295898\\
63	215.279418945313\\
64	214.318267822266\\
65	214.835220336914\\
66	213.944915771484\\
67	214.583953857422\\
68	215.364654541016\\
69	213.991836547852\\
};
\addlegendentry{CF}


\addplot [color=green, mark size=1pt, mark repeat=20, mark=triangle, mark options={solid, fill=green, green}]
table[row sep=crcr]{%
	1	212.048797607422\\
	2	211.445449829102\\
	3	211.121948242188\\
	4	211.119873046875\\
	5	211.677658081055\\
	6	210.939895629883\\
	7	210.494567871094\\
	8	210.619812011719\\
	9	211.110656738281\\
	10	210.578125\\
	11	210.746917724609\\
	12	212.544616699219\\
	13	211.846878051758\\
	14	212.259552001953\\
	15	212.565093994141\\
	16	212.259613037109\\
	17	211.239364624023\\
	18	211.933639526367\\
	19	212.093765258789\\
	20	212.129623413086\\
	21	212.141891479492\\
	22	211.988891601563\\
	23	212.019393920898\\
	24	211.659484863281\\
	25	211.863754272461\\
	26	211.958953857422\\
	27	212.116317749023\\
	28	213.882095336914\\
	29	212.371627807617\\
	30	213.022155761719\\
	31	212.522888183594\\
	32	211.955856323242\\
	33	212.970413208008\\
	34	214.417221069336\\
	35	213.159408569336\\
	36	211.890914916992\\
	37	213.732849121094\\
	38	214.326461791992\\
	39	212.768188476563\\
	40	213.809097290039\\
	41	213.607055664063\\
	42	214.073669433594\\
	43	214.23828125\\
	44	212.786560058594\\
	45	214.552978515625\\
	46	212.588073730469\\
	47	214.45671081543\\
	48	212.524993896484\\
	49	213.913635253906\\
	50	213.791748046875\\
	51	214.068862915039\\
	52	213.183288574219\\
	53	212.819030761719\\
	54	213.396591186523\\
	55	213.826324462891\\
	56	213.698501586914\\
	57	212.469039916992\\
	58	213.198028564453\\
	59	213.004425048828\\
	60	212.766723632813\\
	61	213.797241210938\\
	62	212.636978149414\\
	63	213.822463989258\\
	64	212.592666625977\\
	65	213.298110961914\\
	66	212.142730712891\\
	67	212.811950683594\\
	68	213.752380371094\\
	69	212.366882324219\\
};
\addlegendentry{\textbf{\textcolor{red}{CF-new}}}

\addplot [color=red, dashed, mark size=1pt, mark repeat=20, mark=diamond*, mark options={solid, fill=red, red}]
  table[row sep=crcr]{%
1	212.678636673067\\
2	212.081533850485\\
3	211.706520657107\\
4	211.576598477236\\
5	212.216940467187\\
6	212.811719643296\\
7	212.257102394825\\
8	212.408806805884\\
9	212.81963052383\\
10	212.584945690169\\
11	212.414794720256\\
12	212.969722719366\\
13	212.384525787251\\
14	212.917584941024\\
15	213.109309799076\\
16	213.06583101832\\
17	212.247673588606\\
18	212.489102058275\\
19	213.120724919261\\
20	212.906392935127\\
21	212.776649875951\\
22	212.23550282709\\
23	212.544587946708\\
24	212.00520221087\\
25	212.62499842835\\
26	212.09183014566\\
27	213.016249699094\\
28	213.336153916709\\
29	213.079798383124\\
30	212.968074964886\\
31	213.300937910063\\
32	212.721398188569\\
33	213.082244569721\\
34	213.503241401039\\
35	213.018110462288\\
36	212.618886867997\\
37	213.418348505637\\
38	213.12022734119\\
39	213.169825312232\\
40	213.279503306883\\
41	213.373160752068\\
42	212.98797150193\\
43	213.633194506771\\
44	213.281074271678\\
45	213.515489659923\\
46	213.185239632383\\
47	213.643704858947\\
48	213.121755121527\\
49	212.940016323339\\
50	213.437205827249\\
51	213.499197975139\\
52	212.961470891656\\
53	213.25095957149\\
54	212.719392409096\\
55	213.590036335783\\
56	213.47199759821\\
57	212.806004664008\\
58	213.622311770421\\
59	213.06277421976\\
60	213.374348786559\\
61	212.834109532592\\
62	212.94667028524\\
63	212.9545581961\\
64	213.446419872996\\
65	213.153140084582\\
66	212.98543485395\\
67	213.453018631237\\
68	213.505590605289\\
69	212.922629273901\\
};
\addlegendentry{MPPCA}




\addplot [color=red, line width=1pt, mark size=1pt, mark repeat=20, mark=diamond*, mark options={solid, fill=red, red}]
  table[row sep=crcr]{%
1	212.631131496315\\
2	212.022709620978\\
3	211.65626969339\\
4	211.538052683126\\
5	212.169264775594\\
6	211.750398715815\\
7	211.175662704285\\
8	211.281485961482\\
9	211.813543924595\\
10	211.35591582832\\
11	211.55861125904\\
12	211.317178426623\\
13	210.800195704683\\
14	210.975542072309\\
15	211.683376324681\\
16	211.124899313196\\
17	210.39938815857\\
18	210.555002299601\\
19	211.162100560113\\
20	211.145863408277\\
21	211.224194271944\\
22	211.03685616372\\
23	211.055031128467\\
24	210.847359905858\\
25	211.049573945688\\
26	211.033379978044\\
27	211.419059037515\\
28	211.026161993817\\
29	211.0848679653\\
30	210.369434493427\\
31	211.032873631062\\
32	210.480506504568\\
33	210.568117768886\\
34	211.173987340341\\
35	210.579201411468\\
36	210.408570700374\\
37	210.95250727021\\
38	210.883819740984\\
39	210.723360852733\\
40	210.83445250677\\
41	211.084642045803\\
42	210.590274383942\\
43	211.592394854798\\
44	211.009224421664\\
45	211.316559622806\\
46	211.269477292353\\
47	211.257179803876\\
48	210.638669740349\\
49	210.621474630665\\
50	210.979599305602\\
51	211.392469343866\\
52	210.82952899535\\
53	211.643830240824\\
54	210.396720658305\\
55	211.116043190022\\
56	211.038838420378\\
57	210.336985046334\\
58	211.037181898981\\
59	210.590731431508\\
60	211.42888218287\\
61	210.538591488482\\
62	210.673725189856\\
63	210.737669052138\\
64	211.107728131475\\
65	210.869109092602\\
66	210.400913901394\\
67	210.946168158021\\
68	211.127242123374\\
69	210.579657681555\\
};
\addlegendentry{\textbf{\textcolor{red}{MPPCA-new}}}

\addplot [color=black, dashed, mark size=1pt, mark repeat=20, mark=circle, mark options={solid, fill=black, black}]
table[row sep=crcr]{%
	1	211.615561526927\\
	2	211.018117495868\\
	3	210.786978475474\\
	4	210.546460451446\\
	5	211.169850804282\\
	6	210.325175594885\\
	7	209.868306811864\\
	8	209.914843297849\\
	9	210.570691960018\\
	10	209.956371703603\\
	11	210.190649750467\\
	12	214.911192860516\\
	13	214.524206711469\\
	14	215.445146634253\\
	15	214.145428531696\\
	16	215.487944132157\\
	17	213.650323052506\\
	18	214.742718250031\\
	19	215.102714547207\\
	20	214.493691372191\\
	21	214.275367122479\\
	22	213.391826989346\\
	23	213.723334227498\\
	24	213.063233904889\\
	25	213.937511851463\\
	26	213.526434180438\\
	27	214.203566303696\\
	28	218.411563191577\\
	29	214.471348781741\\
	30	217.194896600826\\
	31	215.120114089706\\
	32	214.621897195799\\
	33	217.317030487585\\
	34	219.311842033125\\
	35	217.358336620497\\
	36	214.65971129239\\
	37	218.280415883217\\
	38	219.196188311709\\
	39	216.107383395443\\
	40	218.383723357645\\
	41	217.259285658185\\
	42	218.723023713173\\
	43	217.451179203082\\
	44	215.450335753574\\
	45	219.499964571289\\
	46	214.529259610177\\
	47	219.097648926544\\
	48	216.148584123684\\
	49	218.691801953417\\
	50	218.114030473723\\
	51	217.405969536075\\
	52	216.761804908223\\
	53	214.606046173058\\
	54	218.058164343067\\
	55	218.023782846913\\
	56	218.116550117162\\
	57	216.261584123853\\
	58	217.062683809088\\
	59	217.143443729149\\
	60	214.786457738823\\
	61	218.376738921246\\
	62	215.708665427355\\
	63	218.46202875897\\
	64	215.383949892661\\
	65	216.92115286139\\
	66	216.096862811322\\
	67	216.491128921322\\
	68	218.153231602589\\
	69	215.410535520958\\
};
\addlegendentry{MAG}


\addplot[area legend, draw=none, fill=mycolor1, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
0	219\\
5.5	219\\
5.5	220\\
0	220\\
}--cycle;
\addlegendentry{$b0$}

\addplot [color=mycolor1, dashdotted, forget plot]
  table[row sep=crcr]{%
5.5	208\\
5.5	220\\
};

\addplot[area legend, draw=none, fill=mycolor2, fill opacity=0.3]
table[row sep=crcr] {%
x	y\\
5.5	219\\
11.5	219\\
11.5	220\\
5.5	220\\
}--cycle;
\addlegendentry{$750\,\text{s/mm}^2$}

\addplot [color=mycolor2, dashdotted, forget plot]
  table[row sep=crcr]{%
11.5	208\\
11.5	220\\
};

\addplot[area legend, draw=none, fill=mycolor3, fill opacity=0.3]
table[row sep=crcr] {%
x	y\\
11.5	219\\
27.5	219\\
27.5	220\\
11.5	220\\
}--cycle;
\addlegendentry{$1500\,\text{s/mm}^2$}

\addplot [color=mycolor3, dashdotted, forget plot]
  table[row sep=crcr]{%
27.5	208\\
27.5	220\\
};

\addplot[area legend, draw=none, fill=mycolor4, fill opacity=0.1]
table[row sep=crcr] {%
x	y\\
27.5	219\\
69	219\\
69	220\\
27.5	220\\
}--cycle;
\addlegendentry{$3000\,\text{s/mm}^2$}

\end{axis}
\end{tikzpicture}%

==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/pc_real/pc_reals2.tex <==

\setlength{\gbarlength}{1.4\iheight}

	\let\iwidth\relax
	\let\iheight\relax
	\let\rowspace\relax
	\newlength{\iwidth}
	\newlength{\iheight}
	\newlength{\rowspace}
	\setlength{\iwidth}{1.4cm}
	\setlength{\iheight}{1.0\iwidth}
	\setlength{\rowspace}{-6pt}
	\setlength{\tabcolsep}{0pt}
	
\tikzset{
	/tpic/options/.style = {
		width=\iwidth,
		height=\iheight,
		scale=1.05,
		xloc=0.5,
		yloc=0.5,
		angle=0,
		color=white,
		label={}
	} 
}
   
\pgfdeclareverticalshading{g1}{.20cm}{ %0.05\colorbarlength
    	rgb(0)=(0,0,0); 
    	rgb(1.30\gbarlength)=(1,1,1)
}    
    
% For two-column wide figures use
\begin{figure}[t]
\centering 	
		\begin{tikzpicture}
		\node(dum) {\subimport{Fig/pc_real/real/}{fig9}};
		\node(cb) [right= -0.5cm of dum] {\gBar{$-20$}{$200$}};
		\end{tikzpicture}
   % \vspace{-1.5\baselineskip} 
   \\
   %\vspace{-5mm} 
    \caption{Phase-corrected DW images ($b=3000\,\text{s/mm}^2$). Red/yellow arrows denote dark holes introduced/mitigated  by conventional/calibrated phase correction.}
	\label{fig4}
\end{figure}



==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/pc_real/real/fig9.tex <==
\tikzset{
		/tpic/options/.style = {
			width =\iwidth,
			height=\iheight,
			scale=1.05,
			xloc=0.5,
			yloc=0.5,
			angle=0,
			color=white,
			label={}
		}
}
\begin{tabular}{ccccccc} 
		%\columnText{$0\,\text{s/mm}^2$}     \tpic[options]{TV}   &  \tpic[options]{TV_real_noise}   &  \tpic[options]{CF}  &  \tpic[options]{CF_real_noise}  & \tpic[options]{MPPCA_real}  & \tpic[options]{MPPCA_real_noise}  &  \tpic[options]{data}  \vspace{-4mm}  \\
		%\columnText{$750\,\text{s/mm}^2$}   \tpic[options]{TV2}  &  \tpic[options]{TV_real_noise2}  &  \tpic[options]{CF2} &  \tpic[options]{CF_real_noise2} & \tpic[options]{MPPCA_real2} & \tpic[options]{MPPCA_real_noise2} &  \tpic[options]{data2} \vspace{-4mm}  \\ 	
		   %\\
		\tpic[options]{TV4}  &  \tpic[options]{TV_real_noise4}  &  \tpic[options]{CF4} &  \tpic[options]{CF_real_noise4} & \tpic[options]{MPPCA4}      & \tpic[options]{MPPCA_real_noise4} &  \tpic[options]{data4} 
		\vspace{-2mm} 
		\\
		\tpic[options]{tv_r}  &  \tpic[options]{tv_n_r}  &  \tpic[options]{cf_r} &  \tpic[options]{cf_n_r} & \tpic[options]{mppca_r} & \tpic[options]{mppca_n_r} &  \tpic[options]{data_r}  
		\vspace{-2mm}
		\\  
		\tiny{TV} &  \tiny{\textbf{\textcolor{red}{TV-new}}}             &  \tiny{CF}     &  \tiny{\textbf{\textcolor{red}{CF-new}}}            & \tiny{MPPCA}          & \tiny{\textbf{\textcolor{red}{MPPCA-new}}}            &  \tiny{MAG}
\end{tabular}



	
%\end{document}


==> Is Perfect Filtering Enough Leading to Perfect Phase Correction_ (Copy)/Fig/pc_real/real2/Fig9a.tex <==
\tikzset{
		/tpic/options/.style = {
			width =\iwidth,
			height=\iheight,
			scale=1.05,
			xloc=0.5,
			yloc=0.5,
			angle=0,
			color=white,
			label={}
		}
}
\begin{tabular}{ccccccc} 
		%\columnText{$0\,\text{s/mm}^2$}     \tpic[options]{TV}   &  \tpic[options]{TV_real_noise}   &  \tpic[options]{CF}  &  \tpic[options]{CF_real_noise}  & \tpic[options]{MPPCA_real}  & \tpic[options]{MPPCA_real_noise}  &  \tpic[options]{data}  \vspace{-4mm}  \\
		%\columnText{$750\,\text{s/mm}^2$}   \tpic[options]{TV2}  &  \tpic[options]{TV_real_noise2}  &  \tpic[options]{CF2} &  \tpic[options]{CF_real_noise2} & \tpic[options]{MPPCA_real2} & \tpic[options]{MPPCA_real_noise2} &  \tpic[options]{data2} \vspace{-4mm}  \\ 	
		   %\\
		\tpic[options]{../real/TV4}  &  \tpic[options]{../real/TV_real_noise4}  &  \tpic[options]{../real/CF4} &  \tpic[options]{../real/CF_real_noise4} & \tpic[options]{../real/MPPCA4}      & \tpic[options]{../real/MPPCA_real_noise4} &  \tpic[options]{../real/data4} 
		\vspace{-2mm} 
		\\
		\tpic[options]{../real/tv_r}  &  \tpic[options]{../real/tv_n_r}  &  \tpic[options]{../real/cf_r} &  \tpic[options]{../real/cf_n_r} & \tpic[options]{../real/mppca_r} & \tpic[options]{../real/mppca_n_r} &  \tpic[options]{../real/data_r}  
		\vspace{-2mm}
		\\  
		\tiny{TV} &  \tiny{\textbf{\textcolor{red}{TV-new}}}             &  \tiny{CF}     &  \tiny{\textbf{\textcolor{red}{CF-new}}}            & \tiny{MPPCA}          & \tiny{\textbf{\textcolor{red}{MPPCA-new}}}            &  \tiny{MAG}
\end{tabular}



	
%\end{document}

